Large-Scale Online Experimentation with Quantile Metrics

Online experimentation (or A/B testing) has been widely adopted in industry as the gold standard for measuring product impacts. Despite the wide adoption, few literatures discuss A/B testing with quantile metrics. Quantile metrics, such as 90th percentile page load time, are crucial to A/B testing as many key performance metrics including site speed and service latency are defined as quantiles. However, with LinkedIn's data size, quantile metric A/B testing is extremely challenging because there is no statistically valid and scalable variance estimator for the quantile of dependent samples: the bootstrap estimator is statistically valid, but takes days to compute; the standard asymptotic variance estimate is scalable but results in order-of-magnitude underestimation. In this paper, we present a statistically valid and scalable methodology for A/B testing with quantiles that is fully generalizable to other A/B testing platforms. It achieves over 500 times speed up compared to bootstrap and has only $2\%$ chance to differ from bootstrap estimates. Beyond methodology, we also share the implementation of a data pipeline using this methodology and insights on pipeline optimization.

==> comments.tex <==

\citep{box2005statistics,gerber2012field}, has gained popularity as the gold standard for evaluating new product ideas across industry. Many companies have built in-house A/B testing platforms to meet their complex experimentation needs. Some have been discussed at length in past papers \citep{tang2010overlapping, kohavi2013online, bakshy2014designing, xu2015}, including best practices and pitfalls \citep{kohavi2012trustworthy, dmitriev2017dirty}. While the number of metrics have grown to 3000+, 

At LinkedIn, A/B testing is at the core of data driven decision making. To facilitate better decision making, we monitor over 3000 metrics in each A/B test, ranging from company-wide true north metrics such as revenue and daily active users, to much more granular product line specific use engagement metris. (cite Bonnie's blogpost). Most metrics are averages, and average is okay in most cases, for example, total revenue is simply average revenue times number of people. For performance metrics, however, quantile is needed. Quantile metrics are a very important type of metrics. For example, one of our company top-line metric, 90th percentile sitespeed (or p90 sitespeed) is a quantile. With performance metrics, average is not representative. As an example, imagine two websites with the same average pageLoadTime 0.5 seconds. Site A loads every singel page with 0.5 seconds and would be perceived as a fast site

There are many strategies to grow page views, as two examples, you can either revive dormant users, or encourage already active users to be even more active. Although both strategies may result in the same growth of page views, one strategy may be more sustainable than the other. If your site is such that once a user becomes active they will stay active with high probability, then focusing on  often 

If your site is such that once a user becomes active they will stay active with high probability, then focusing on  often  For example, LinkedIn creates economic opportunities for professionals partly through connecting them to other professionals. While we  Other use cases include measuring fairness. For example, if we grow the average connections in the ecosystem by $5\%$, do we achieve that by making every one more connected, or making the already well-connected even more connected? It is also applicable outside LinkedIn. For example, in a rideshare system, it would be very important to control the worst waiting time, riders would be happy to wait 2 minute longer for every ride, but they might not be happy to allow one of ten rides to take 20 mins longer.

we present a statistically valid and scalable methodology for A/B testing with quantiles that is fully generalizable to other A/B testing platforms. It achieves over 500x speed up compared to bootstrap and has only $2\%$ chance to differ from bootstrap estimates. Beyond methodology, we also share the implementation of a data pipeline using this methodology and insights on pipeline optimization.



 

. Despite their importance, quantile metrics have not been supported in the reporting and experimentation ecosystem due to the high cost to estimate p-values for them. The quantiles pipeline would take over 4 months to compute p-values for all p90 sitespeeds on all testkeys. In comparison, the xlnt-full pipeline, which ingests 40 times more metrics, completes in merely 4 hours. 



of However, there is no existing literature on how to efficiently estimate variance of quantiles when each measurement is not mutually independent, which is the distribution that our pageLoadTimes(plt) fit into. For example, plt’s from the same user are not independent. 
The major challenge in this project is therefore, to research and design an algorithm that efficiently computes variance of quantiles when samples are NOT independent.

\subsection{Existing Solutions}
There are two existing methodologies for quantile standard deviation estimates, neither of with are both statistically valid and scalabel. They are 1. the classical asymptotic estimate which assumes page load times $X_{i,j}$ are i.i.d; 2. bootstrap which does not necessarily assume samples are \textit{i.i.d.}. By resampling on members instead of page views, bootstrap can preserve the dependence structure in the data, therefore results in valid estimates of standard deviation. The downside of bootstrap is however, it is not scalable due to the need to compute quantiles on thousands of resamples. 

\begin{references}
\itemsep=0pt
{\footnotesize
\item 
Box, G. E., Hunter, J. S., Hunter, W. G. (2005), {\it Statistics for
experimenters: design, innovation, and discovery}, Vol. 2., Wiley-Interscience New
York.

\item 
Gerber, A. S., and Green, D. P. (2012), {\it Field experiments: design, analysis, and
interpretation}, WW Norton.

\item 
Alerstam, T. (1990), {\it Bird Migration}, Cambridge, UK: Cambridge University Press.
Henning Hohnhold, Deirdre O’Brien, and Diane Tang. 2015. Focusing on the
Long-term: It’s Good for Users and Business. In Proceedings of the 21th ACM
SIGKDD International Conference on Knowledge Discovery and Data Mining. ACM,
1849–1858



\item 
Berthold, P. (2001), {\it Bird Migration: A General Study} (2nd ed.), Oxford, UK: Oxford University Press.

\item 
Booth, J., and Hobert, J. P. (1999), ``Maximizing Generalized Linear Mixed Model Likelihoods With an Automated Monte Carlo EM Algorithm,'' {\it Journal of the Royal Statistical Society}, Ser. B, 61, 265--285.

\item 
Burnham, K. P., and Anderson, D. R. (1998), {\it Model Selection and Inference}, New York: Springer.

\item 
Cerioli, A. (1997), ``Modified Tests of Independence in $2 \times 2$ Tables With Spatial Data,'' {\it Biometrics}, 53, 619--628.

\item
Chan, J. S. K., and Kuk, A. Y. C. (1997), ``Maximum Likelihood Estimation for Probit-Linear Mixed Models With Correlated Random Effects,'' {\it Biometrics}, 53, 86--97. 

\item
Chen, J., Zhang, D., and Davidian, M. (2002), ``A Monte Carlo EM Algorithm for Generalized Linear Mixed Models With Flexible Random Effects Distribution,'' {\it Biostatistics}, 3, 347--360.

\item
Chib, S. (1995), ``Marginal Likelihood From the Gibbs Output,'' {\it Journal of the American Statistical Association}, 90, 1313--1321.

\item
Cooper, A. B., and Millspaugh, J. J. (1999), ``The Application of Discrete Choice Models to Wildlife Resource Selection Studies,'' {\it Ecology}, 80, 
566--575.

\item
Dempster, A. P., Laird, N. M., and Rubin, D. B. (1977), ``Maximum Likelihood From Incomplete Data via the EM Algorithm,'' {\it Journal of the Royal Statistical Society}, Ser. B, 39, 1--38.

\item
Erickson, W. P., McDonald, T. L., Gerow, K. G., Howlin, S., and Kern, J. W. (2001), ``Statistical Issues in Resource Selection Studies With Radio-marked Animals,'' in {\it Radio Telemetry and Animal Populations}, eds. J. Millispaugh and J. Marzluff, California: Academic Press, pp. 209--242.

}
\end{references}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{ind_vs_bootstrap.eps}
        \caption{Asymptotic estimate assuming independence}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{proposed_vs_bootstrap.eps}
        \caption{Proposed estimate}
    \end{subfigure}
    \caption{Proposed VS. Existing Method}
\end{figure}  
